LeTS-Drive: Driving in a Crowd by Learning from Tree Search

Autonomous driving in a crowded environment, e.g., a busy traffic intersection, is an unsolved challenge for robotics. The robot vehicle must contend with a dynamic and partially observable environment, noisy sensors, and many agents. A principled approach is to formalize it as a Partially Observable Markov Decision Process (POMDP) and solve it through online belief-tree search. To handle a large crowd and achieve real-time performance in this very challenging setting, we propose LeTS-Drive, which integrates online POMDP planning and deep learning. It consists of two phases. In the offline phase, we learn a policy and the corresponding value function by imitating the belief tree search. In the online phase, the learned policy and value function guide the belief tree search. LeTS-Drive leverages the robustness of planning and the runtime efficiency of learning to enhance the performance of both. Experimental results in simulation show that LeTS-Drive outperforms either planning or imitation learning alone and develops sophisticated driving skills.

==> diff <==
Index: RSS2019Cai.tex
===================================================================
--- RSS2019Cai.tex	(revision 3728)
+++ RSS2019Cai.tex	(revision 3729)
@@ -733,13 +733,14 @@
 
 
 \section{Conclusion}
+
 This work addresses the challenge of autonomous driving among many                                   
 pedestrians. \letsdrive leverages the robustness of planning and the runtime                        
 efficiency of learning. It integrates them to advance the performance of                            
 both. \letsdrive applies a two-stage approach. It learns a policy by imitating                      
 the belief tree search and then guides the belief tree search using the                             
-learned policy and its value function. \letsdrive outperforms planning and                          
-learning approaches significantly in both safety and efficiency, and                                
+learned policy and its value function. \letsdrive outperforms the planning or the                         
+learning approach alone in both safety and efficiency, and                                
 demonstrates sophisticated driving behaviors in simulation. 
 % This paper addressed the problem of driving among a crowd of pedestrians, and proposed \letsdrive, that solves this extremely large-scale problem by integrating POMDP planning and deep learning. \letsdrive leverages the robustness of planning and the runtime efficiency of learning and integrates them to advance the performance of both. It applies a two-stage approach: learning a policy by imitating the belief tree search, and guiding the belief tree search using the learned policy and its value function. \letsdrive outperforms planning and learning approaches significantly in both safety and efficiency, and demonstrates sophisticated driving behaviors in simulation.  
 
@@ -747,10 +748,13 @@
 % Main limitations of the work include two aspects. First, the amount of online search is constrained by the complexity of the neural networks. To further improve the performance, we need to investigate more efficient representations of the policy and the value.
 {\color{blue}There are two main limitations in our current work. First,                             
 the efficiency of online search is constrained by the complexity of the                         
-learned  neural networks. To further improve the performance, we plan to                            
-investigate more efficient representations of the policy and the value functions.                    
+learned  neural networks. To further improve performance, we plan to                            
+investigate more efficient policy and value function representations.                    
 % Second, while integration with deep learning breaks the theoretical guarantee of HyP-DESPOT, it improves the practical performance significantly in both training and testing maps. To further generalize to complex real-world environments, we will develop richer, better-randomized simulations with more sophisticated motion models for both pedestrians and vehicles. 
-Second, integration with deep learning challenges the generalization to prominently different maps and crowd types. To address this, we plan to improve the training environment with rich real-world maps and more sophisticated motion models to simulate diverse agents.
+Second, it remains  a  challenge to generalize the learned policies
+and value functions over diverse maps and
+agent behaviors.  We plan to expand the training environment with rich
+real-world maps and more sophisticated agent motion models.
 % Second, integration with deep learning breaks the theoretical guarantee of HyP-DESPOT, but improved the practical performance significantly in both training and testing maps. To further generalize to complex real-world environments, we will develop richer, better-randomized simulations with more sophisticated motion models for both pedestrians and vehicles.  
 % Importantly, \letsdrive can be extended to perform general reinforcement learning by building a closed loop between the imitation and the improvement stages. In principle, we can use the improved policy as the expert for the next imitation stage, and execute the loop iteratively. By doing so, \letsdrive will improve the learned policy and the guided search simultaneously with the increasing amount of data. This will be the focus of our future work. 
 }


==> settings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2345678901234567890123456789012345678901234567890123456789012345678901234567890
%        1         2         3         4         5         6         7         8

% Enable PDF 1.7 output 
\pdfminorversion = 7
% Suppress the pdf group warning
\usepackage{authblk}
\usepackage[a4paper, left=0.6in, right=0.6in, top=1in, bottom=0.8in]{geometry}
\setlength{\columnsep}{0.3in}

\usepackage{times}

% numbers option provides compact numerical references in the text. 
\usepackage[numbers,sort&compress]{natbib}
% \usepackage{multicol}
\usepackage[bookmarks=true]{hyperref}

\pdfinfo{
   /Author (Panpan Cai, Yuanfu Luo, David Hsu and Wee Sun Lee)
   /Title  (HyP-DESPOT)
   /CreationDate (D:)
   /Subject (Planning under uncertainty)
   /Keywords (Planing under uncertainty;Parallel POMDP planning)
}


\usepackage{pdfsync}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\usepackage{graphicx}
  \graphicspath{{Figures/}}
  \DeclareGraphicsExtensions{.pdf,.jpg,.png,.eps}
\usepackage{pdfpages}
\usepackage{bm}
\usepackage{amsmath,amssymb}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
%\usepackage{cite}
\usepackage{xspace}
\usepackage{booktabs}
\usepackage{amsthm}
%\usepackage{soul}
%\usepackage{microtype}
\usepackage[toc,page]{appendix}

%% references
\newcommand{\secref}[1]{Section~\ref{#1}}
\renewcommand{\eqref}[1]{(\ref{#1})}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\subfigref}[1]{Fig.~\subref*{#1}}

\newcommand{\subfig}[1]{\textit{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}

%% abbreviations
\newcommand{\ie}{\textrm{i.e.}}
\newcommand{\eg}{\textrm{e.g.}}
\newcommand{\etc}{\textrm{etc.}}
\newcommand{\etal}{\textrm{et~al.}}

%% math
\newtheorem{theorem}{Theorem}

\newenvironment{dm}
  {\vspace*{-2pt}\displaymath}{\vspace*{-2pt}\enddisplaymath}
\newenvironment{eq}
  {\vspace*{-2pt}\equation}{\vspace*{-2pt}\endequation}
\newcommand{\sss}{\scriptscriptstyle}

\DeclareMathOperator*{\argmax}{arg\,max} % Jan Hlavacek
\newcommand{\mean}{\ensuremath{\mathbb{E}}\xspace}
\newcommand{\pr}{\ensuremath{p}}

%% citation
\newcommand{\tinylineskip}{\baselineskip=4pt}
\newlength{\citeskipup}
\newlength{\citeskipdown}
\newcommand{\citeinfo}[2]{{\footnotesize \tinylineskip
  \vspace*{\citeskipup}\noindent {\sc #1} \\
  {#2} \vspace*{\citeskipdown}}}

%% comment
\usepackage{color}
% \definecolor{darkgreen}{rgb}{0,0.5,0} 
\definecolor{fullred}{rgb}{0.95,.0,.1} 
% \definecolor{brown}{rgb}{0.65,0.16,0.16} 
% \definecolor{orange}{rgb}{1,0.5,0} 
\setlength{\marginparwidth}{0.5in}
\newcounter{cmt}
\newcommand{\comment}[2]{\addtocounter{cmt}{1} {\color{fullred} #1}\marginpar{\tiny\noindent{\raggedright{\color{fullred}[\arabic{cmt}]}\newline\color{fullred}{#2} \par}}}

%% make a thick line in tables using double rules
%\setlength{\doublerulesep}{\arrayrulewidth}



\newcommand{\freq}{\ensuremath{N}\xspace}
\newcommand{\freqsymbol}{\ensuremath{N}}
\newcommand{\nscen}{\ensuremath{K}\xspace}
\newcommand{\nscensymbol}{\ensuremath{K}}
\newcommand{\scenario}{\ensuremath{{\boldsymbol{\phi}}}\xspace}
\newcommand{\scenarioset}{\ensuremath{{\boldsymbol{\Phi}}}\xspace}
\newcommand{\scenariosetnode}[1]{\ensuremath{{\boldsymbol{\Phi}_{#1}}}\xspace}
\newcommand{\scenariosetsize}[1]{\ensuremath{|\scenariosetnode{#1}|}\xspace}

\newcommand{\randnum}{\ensuremath{\varphi}\xspace}

\newcommand{\state}{\ensuremath{s}\xspace}
\newcommand{\scurr}{\ensuremath{s}\xspace}
\newcommand{\snext}{\ensuremath{s'}\xspace}
\newcommand{\obs}{\ensuremath{z}\xspace}
\newcommand{\act}{\ensuremath{a}\xspace}
\newcommand{\reward}{\ensuremath{r}\xspace}
\newcommand{\optact}{\ensuremath{a^*}\xspace}
\newcommand{\optobs}{\ensuremath{z^*}\xspace}
\newcommand{\obsprob}[3]{\ensuremath{O({#1},{#2},{#3})}\xspace}
\newcommand{\obsfun}{\ensuremath{O}\xspace}
\newcommand{\transfun}[3]{\ensuremath{T({#1},{#2},{#3})}\xspace}
\newcommand{\obsprobsym}{\ensuremath{O}\xspace}
\newcommand{\transfunsym}{\ensuremath{T}\xspace}
\newcommand{\rfun}[2]{\ensuremath{R({#1},{#2})}\xspace}
\newcommand{\rfunsymbol}{\ensuremath{R}\xspace}
\newcommand{\rmax}{\ensuremath{R_{max}}\xspace}

\newcommand{\stateset}{\ensuremath{S}\xspace}
\newcommand{\obsset}{\ensuremath{Z}\xspace}
\newcommand{\actset}{\ensuremath{A}\xspace}
\newcommand{\sinit}{\ensuremath{s_0}\xspace}
\newcommand{\elementset}{\ensuremath{E}\xspace}

\newcommand{\belief}{\ensuremath{b}\xspace}
\newcommand{\node}{\ensuremath{b}\xspace}
\newcommand{\newbelief}{\ensuremath{b'}\xspace}
\newcommand{\newnode}{\ensuremath{b'}\xspace}
\newcommand{\leafnode}{\ensuremath{b}\xspace}
\newcommand{\rootnode}{\ensuremath{b_0}\xspace}
\newcommand{\pol}{\ensuremath{\pi}\xspace}
\newcommand{\polset}{\ensuremath{\Pi}\xspace}
\newcommand{\defaultpol}{\ensuremath{\pi_0}\xspace}

\newcommand{\polvalue}{\ensuremath{V}\xspace}
\newcommand{\nodevalue}{\ensuremath{v}\xspace}
\newcommand{\optnodevalue}{\ensuremath{v^*}\xspace}

\newcommand{\ascale}{\ensuremath{c_a}\xspace}
\newcommand{\oscale}{\ensuremath{c_o}\xspace}

\newcommand{\timestep}{\ensuremath{t}\xspace}
\newcommand{\depth}{\ensuremath{\Delta}\xspace}
\newcommand{\maxsearchdepth}{\ensuremath{D}\xspace}
\newcommand{\nvisit}[1]{\ensuremath{N({#1})}\xspace}
\newcommand{\nvisita}[2]{\ensuremath{N({#1},{#2})}\xspace}
\newcommand{\ubsymbol}{\ensuremath{u}\xspace}
\newcommand{\ub}[1]{\ensuremath{\ubsymbol({#1})}\xspace}
\newcommand{\uba}[2]{\ensuremath{\ubsymbol({#1},{#2})}\xspace}
\newcommand{\iniub}[1]{\ensuremath{\ubsymbol_0({#1})}\xspace}
\newcommand{\lbsymbol}{\ensuremath{l}\xspace}
\newcommand{\lb}[1]{\ensuremath{\lbsymbol({#1})}\xspace}
\newcommand{\inilb}[1]{\ensuremath{\lbsymbol_0({#1})}\xspace}
\newcommand{\gap}[1]{\ensuremath{\epsilon({#1})}\xspace}
\newcommand{\gapsymbol}{\ensuremath{\epsilon}\xspace}

\newcommand{\augub}[2]{\ensuremath{u^{+}({#1},{#2})}\xspace}
\newcommand{\augweu}[1]{\ensuremath{E^{+}({#1})}\xspace}
\newcommand{\weu}[1]{\ensuremath{E({#1})}\xspace}
\newcommand{\vloss}{\ensuremath{\zeta}\xspace}
\newcommand{\dsmodelf}[3]{\ensuremath{g({#1},{#2},{#3})}\xspace}
\newcommand{\dsmodel}{\ensuremath{g}\xspace}
\newcommand{\beliefupdate}{\ensuremath{\tau}\xspace}
\newcommand{\online}{{online}\xspace}
\newcommand{\offline}{{offline}\xspace}
\newcommand{\rollout}{{roll-out}\xspace}
%\newcommand{\forall}{\text{for all }\xspace}


\newcommand{\accel}{{\small \textsc{Accelerate}}}
\newcommand{\decel}{{\small \textsc{Decelerate}}}
\newcommand{\maintain}{{\small \textsc{Maintain}}}
\newcommand{\sample}{{\small \textsc{Sample}}\xspace}
\newcommand{\sense}{{\small \textsc{Sense}}\xspace}
\newcommand{\good}{{\small \textsc{Good}}\xspace}
\newcommand{\bad}{{\small \textsc{Bad}}\xspace}

\newcommand{\occupied}{{\small \textsc{Occupied}}\xspace}
\newcommand{\free}{{\small \textsc{Free}}\xspace}

% \newcommand{\element}{within-step\xspace}
% \newcommand{\elementlevel}{within-step\xspace}
% \newcommand{\Elementlevel}{Within-step\xspace}

\newcommand{\element}{factored-model\xspace}
\newcommand{\elementlevel}{factored-model level\xspace}
\newcommand{\Elementlevel}{Factored-model level\xspace}

\newcommand{\RockSample}{Rock Sample\xspace}
\newcommand{\RockSampleTight}{Rock Sample}
%\documentclass[a4paper, 10pt, conference]{ieeeconf}      % Use this line for a4 paper

%\IEEEoverridecommandlockouts                              % This command is only needed if 
                                                          % you want to use the \thanks command

%\overrideIEEEmargins                                      % Needed to meet printer requirements.

\setlength{\belowcaptionskip}{-10pt}


\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}

\newcommand{\hyptree}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\thread}{\ensuremath{\psi}\xspace}
\newcommand{\threadset}{\ensuremath{\Psi}\xspace}
\newcommand{\threadnum}{\ensuremath{N}\xspace}
\newcommand{\optthread}{\ensuremath{\tilde{\psi}}\xspace}

\newcommand{\maxexploretime}{\ensuremath{\delta T}\xspace}
\newcommand{\maxexpandtime}{\ensuremath{\delta T_e}\xspace}
\newcommand{\maxforwardtime}{\ensuremath{\delta T_f}\xspace}
\newcommand{\maxbackuptime}{\ensuremath{\delta T_b}\xspace}

\newcommand{\nonexpandduration}{\ensuremath{\delta T'}\xspace}


